More Than Just Warnings:Exploring the Ways of Communicating Credibility Assessment on Social Media

Reducing the spread of misinformation is challenging. AI-based fact verification systems offer a promising solution by addressing the high costs and slow pace of traditional fact-checking. However, the problem of how to effectively communicate the results to users remains unsolved. Warning labels may seem an easy solution, but they fail to account for fuzzy misinformation that is not entirely fake. Additionally, users' limited attention spans and social media information should be taken into account while designing the presentation. The online experiment (n = 537) investigates the impact of sources and granularity on users' perception of information veracity and the system's usefulness and trustworthiness. Findings show that fine-grained indicators enhance nuanced opinions, information awareness, and the intention to use fact-checking systems. Source differences had minimal impact on opinions and perceptions, except for informativeness. Qualitative findings suggest the proposed indicators promote critical thinking. We discuss implications for designing concise, user-friendly AI fact-checking feedback.

==> itroversion.tex <==
Social media platforms like Facebook, Twitter, Reddit, WhatsApp, and TikTok have emerged as primary online locations for people to seek and share information. However, this has been accompanied by a significant increase in the spread of misinformation. Online misinformation includes posts, re-posts, or statements that are misleading due to inaccurate, incorrect, or biased content, regardless of being part of any deliberate plan to deceive for a specific objective or propaganda.\footnote{This latter is called disinformation, see for instance, CISA's \url{https://www.cisa.gov/topics/election-security/foreign-influence-operations-and-disinformation}}
To comply with regulations \footnote{ \url{https://www.cima.ned.org/publication/chilling-legislation/}} and provide better services to their users, social media platforms are trying to reduce the spread of misinformation. To achieve this goal, they implemented a range of solutions to identify the questionable content. One solution is to implement measures that concentrate on reducing content visibility (up to complete deletion) \cite{zeng2022content,gillespie2022not}.Another solution is to actively collaborate with independent fact-checker organizations\cite{facebookIntoFacebook,tiktokCombatingMisinformation}, who, using the practices of journalists' investigation, make the analysis of the claims and provide the verdict.

However, it is widely reported that fact-checking is labor-intensive and often not timely, with results frequently appearing days later. Additionally, only a small portion of the content is fact-checked. Therefore, automatic credibility assessment methods powered by Machine Learning(ML) and Artificial Intelligence(AI) have been increasingly explored. The implementation of AI-based fact-checking instruments can significantly increase the efficiency and coverage of the procedure. The modern AI-based methods can step-by-step imitate the procedures and steps that are taken by human fact-checkers, including claim detection, evidence retrieval, verdict prediction, and justification procedures  \cite{guo2022survey}; moreover, it can create an opportunity to produce detailed (not just true/false) ratings of credibility using the big range of sources and attending the weights to different parameters of information \cite{guo2022survey}. As parameters of information that can be used as the reason for verification in automated scenarios, several papers mention the use of cues from the verified text (like emotions \cite{liu2024emotion} or text coherence with existing "approved" knowledge bases like Wikipedia \cite{thorne2018fever}, but also the extra-textual external cues about the information like source reputation \cite{pillai2024hierarchical} and social clues like likes and reposts (e.g. \cite{yang2019unsupervised} similarly to the strategies performed by fact-checkers (ref) and users \cite{tang2024knows}.

While progress has been made in detection and verification, effectively communicating the results of AI-based fact-checking to users remains an open challenge\cite{guo2022survey}, which requires rethinking the current approaches to interacting with users.

Currently, social media platforms mainly signal the fact-checking results through warning labels, which inform users about identified problems with the content\cite{lim2023effects}. Yet, while studies showed that these measures inform users about misinformation  \cite{martel2023misinformation,mende2024fighting}, several concerns might affect their efficiency. One concern is the complex nature of online misinformation, which often cannot be neatly categorized as either true or false \cite{martel2023misinformation}. 
This complexity can arise either from conflicting evidence or from blending factual information with personal opinions and experiences in posts \cite{zhao2021detecting,li2022health,krause2022infodemic}. However, current labels usually mark content as false, therefore oversimplifying the issue and provoking questions about their trustworthiness \cite{stomber2021towards}. Another issue is that current indicators give users little insight into why content is marked as false. For example, platforms use warning flags referencing third-party fact-checkers \cite{brandtzaeg2016emerging}. However, these fact-checker findings are typically hosted on separate websites, not adjacent to the flagged material. 
This means users must take extra steps to find the information they need, making the process long and complicated \cite{tang2024knows}. As a result, users may not understand who these fact-checkers are \cite{kirchner2020countering} and might end up simply trusting or distrusting an indicator without digging into the reasons based on which the claim was made. Several studies showed that an explanation of the reasons near the warning labels could help users make a decision about information veracity \cite{epstein2022explanations,martel2023misinformation}; however, which type of information should be put inside these labels requires future exploration \cite{spradling2021protection}. 

To better communicate the results of the AI fact-checking system to users, we should avoid the problems associated with the current warning system listed above. Additionally, the solutions should take into account the context in which misinformation appears on social media. Due to information overload on social media, users often make quick decisions and do not always want to engage deeply with the content and debunking messages\cite{talwar2019people}. This means that explanation modes involving long and detailed text will probably not be applicable in scenarios where the person does not have the time or inclination to engage with it, leading to the need to present information in a condensed way that still provides users with enough content for reasoning and decision-making.

In the present paper, we investigate several ways to enhance the communication of post veracity via understanding which information should be included in AI-based fact-checking and  misinformation warning systems. We look into what works better in warning users and what information a future misinformation warning system should report to users.
We conducted a pre-registered, human-subject experiment with 537 participants, drawing upon literature on interface cues and decision support systems in misinformation evaluation. 
We simulated scenarios in which individuals read and assessed the veracity of information. We then varied the sources of credibility—either content-based (internal) or extra-content-based (external)—and the system's indication of veracity, presenting the probability of information being true or false, rather than a binary true/false indication. This experiment explore how these conditions affect users' judgments of news credibility and their trust in AI-driven fact-checking aids.

We found both internal and external credibility indicators significantly aid users in evaluating the truthfulness of information without notable differences in opinion changes, system competence, and trust levels, except for informativeness. This underscores the value of certain meta information in veracity judgments, especially in environments like encrypted messaging platforms where direct content assessment is not feasible. Furthermore, we found fine-grained indicators can provide more nuanced opinions, empowering users to make informed decisions about the content they encounter. We also discovered that the granularity of these indicators and the certainty they convey significantly affect user experience and perceptions of information veracity, highlighting their potential in scenarios where information is not fully verified. Finally, we found the explanations constructed around these indicators enhance critical thinking, encouraging users to reassess information based on the credibility cues provided, thereby promoting a more critical engagement with content.

Our contributions are as follows:
\begin{itemize}
    \item We have undertaken a comprehensive examination of how a system's assessment of social media post veracity influences users' perceptions of its credibility. This analysis helps in understanding the interplay between automated veracity checks and user trust.
    \item We provide an analysis of how the non-binary indicators of content veracity and sources of system's opinion about veracity shape users opinion about information credibility.
    \item We demonstrate that systems informing users about the trustworthiness of information (beyond simply flagging false information) are perceived as valuable. Our research provides evidence of how such systems could assist users in developing a more nuanced approach to trusting online information.
    \item We discuss emerging trends in the realm of information veracity-checking systems and propose design recommendations based on our findings. These recommendations aim to enhance the effectiveness and user-friendliness of future systems, contributing to a more informed and discerning online community.
\end{itemize}

%Due to progress in Machine Learning and AI, AI can now be used to combat online misinformation. For example, it is widely reported that fact-checking is labor-intensive and often not timely, with results frequently appearing days later. Additionally, only a small portion of the content is fact-checked. Therefore, 


%Several studies dedicated to the development of AI-powered explanatory systems also showed that users are taking the system explanations (in the narrative form) into account while assessing the information.

%However, in the context of combatting misinformation in social media, where the stakes of the information are usually low and the user's attention is limited, it is also important to explore the short modes of providing the outcomes of AI-system credibility estimates that still can give the user enough content for reasoning and decision-making.

%social media platforms implement measures that concentrate either on reducing content visibility (up to the complete deletion) \cite{zeng2022content,gillespie2022not} or communicating with the users by cues. The most common cues are warning labels, which inform users about the identified problems with the content, mostly based on the results of the third-party fact-checkers' work \cite{lim2023effects}.

==> lib/macro.tex <==
%% commenting
\usepackage{soul}
\usepackage{xspace}

\newtoggle{comments}
\newtoggle{draft}

\newcommand{\fixit}[1]
{\iftoggle{comments}
{\textcolor{red!70!}{{[$\longleftarrow$\hl{\textbf{FIX!}}]}}
{\marginnote{\huge\textcolor{red}{$\times$}}}}
{}}

\newcommand{\gl}[1]
{\iftoggle{comments}
{~\textcolor{blue!70!}{$^{(\textbf{gl})}~\!\!\leftarrow${[\hl{#1}]}}}
{}}

\newcommand{\guest}[1]
{\iftoggle{comments}
{~\textcolor{gray!90!}{$^{(\textbf{guest})}~\!\!\leftarrow$ {[\hl{#1}]}}}
{}}

\newcommand{\note}[1]
{\iftoggle{draft}
{\noindent\textcolor{red}
{$\triangleright$}$\rightarrow$\hl{\emph{#1}}
$\leftarrow$\textcolor{red}{$\triangleleft$}}
{}}

%%%%%%%%%%%%%
%% short cuts

%% maths
\newcommand{\fun}[1]{\mathtt{#1}}
\newcommand{\mat}[1]{\mathit{#1}}
\newcommand{\set}[1]{\{#1\}}

%% names
\newcommand{\gabriele}{Gabriele Lenzini}

\newcommand{\gab}{\gabriele}

%%  editing macro
\newcommand{\ie}{\emph{i.e.},\xspace}
\newcommand{\eg}{\emph{e.g.},\xspace}
\newcommand{\etal}{\emph{et al.}\xspace}

%% theorem like environments
\newtheorem{thrm}{Theorem}[section]
\newtheorem{lemm}[thrm]{Lemma}
\newtheorem{prop}[thrm]{Proposition}
\newtheorem{crll}{Corollary} 
\newtheorem{defn}{Definition} 
\newtheorem{exmp}{Example}

